Has the Creativity of Large-Language Models peaked? An analysis of inter- and intra-LLM variability

Following the widespread adoption of ChatGPT in early 2023, numerous studies reported that large language models (LLMs) can match or even surpass human performance in creative tasks. However, it remains unclear whether LLMs have become more creative over time, and how consistent their creative output is. In this study, we evaluated 14 widely used LLMs -- including GPT-4, Claude, Llama, Grok, Mistral, and DeepSeek -- across two validated creativity assessments: the Divergent Association Task (DAT) and the Alternative Uses Task (AUT). Contrary to expectations, we found no evidence of increased creative performance over the past 18-24 months, with GPT-4 performing worse than in previous studies. For the more widely used AUT, all models performed on average better than the average human, with GPT-4o and o3-mini performing best. However, only 0.28% of LLM-generated responses reached the top 10% of human creativity benchmarks. Beyond inter-model differences, we document substantial intra-model variability: the same LLM, given the same prompt, can produce outputs ranging from below-average to original. This variability has important implications for both creativity research and practical applications. Ignoring such variability risks misjudging the creative potential of LLMs, either inflating or underestimating their capabilities. The choice of prompts affected LLMs differently. Our findings underscore the need for more nuanced evaluation frameworks and highlight the importance of model selection, prompt design, and repeated assessment when using Generative AI (GenAI) tools in creative contexts.

==> Intro_9_sentences.tex <==
\section{Introduction}
%General Context:
Recent advances in artificial intelligence have challenged long-standing assumptions about human creativity as a uniquely human trait.

%Specific Context:
Large Language Models (LLMs) such as GPT-4, Claude, Gemini, and Mistral now generate ideas, texts, and concepts that often appear indistinguishable from human output.

%Prior Research and Open Questions:
Previous research on generative AI has demonstrated that LLMs can perform well in standardized creativity tests, such as the Divergent Association Task (DAT) and the Alternative Uses Task (AUT), sometimes matching or exceeding human performance.

%Research Gap:
Despite these findings, key questions remain: How do current state-of-the-art LLMs compare in terms of creative potential, and which model is best suited for creative tasks? Additionally, does a given LLM provide diverse ideas within a single session, or does it streamline responses toward a narrow set of outputs?

%Study Aim:
This study aims to assess both the overall creative capacity of contemporary LLMs and the internal variance of their outputs to determine whether they foster idea diversity or converge on repetitive thinking.

%Methodology:
We systematically evaluate a diverse set of LLMs using the DAT and AUT, applying standardized creativity assessment frameworks while tracking both inter-model differences (creativity across models) and intra-model variance (creativity within repeated interactions with the same model).

%Comparative Analysis:
By analyzing originality, fluency, and semantic diversity, we determine which LLMs perform best in generating creative ideas and how consistently they maintain diversity in their outputs.

%Contribution to AI Creativity Debate:
Our findings contribute to the ongoing debate on artificial creativity, addressing both the practical question of selecting the best LLM for creative tasks and the theoretical implications of whether these models enhance or limit divergent thinking.

%Significance of the Study:
By revisiting and expanding previous research, this study provides a comprehensive evaluation of LLM creativity, offering insights into their evolving role as tools for human ideation and problem-solving.


==> Old_stuff.tex <==
\begin{comment}
\section{Creativity of Large Language Models}

Creativity has long been considered a uniquely human trait, distinguishing us from machines and automation. However, recent advances in generative artificial intelligence (GenAI) have reignited debates about whether AI can exhibit creativity, particularly in fields such as literature, music, art, and problem-solving. While AI has already surpassed human capabilities in structured domains like chess and Go \citep{miller_artist_2019}, it remains uncertain whether it can achieve true creativity or if it simply recombines existing knowledge in novel ways \citep{holford_future_2019, kirkpatrick_can_2023, white_opinion_2023}. This section overviews how LLMs perform on creativity-related tasks and how their outputs compare to human-generated content.

Theoretical perspectives define creativity as the ability to generate \textit{new} and \textit{useful} ideas \citep{runco_standard_2012, plucker_generalization_2004}. Creativity is often conceptualized as an interaction between cognitive abilities, environmental factors, and social validation \citep{amabile_pursuit_2017, noauthor_richards_nodate}. High-level creativity, particularly in science and the arts, requires not only originality but also refinement, testing, and evaluation \citep{benedek_motives_2020, kaufman_creative_2016, simonton_what_2013}. While human creativity involves free-associative thinking and problem formulation \citep{steele_looking_2018, botella_what_2018}, GenAI mimics these processes through probabilistic text generation and pattern recognition \citep{marcus_very_2022}.

Recent research suggests that GenAI can support human creativity by recombining existing knowledge in novel ways \citep{cope_computer_2005, reddy_artificial_2022}. In fields such as literature, GenAI-generated text often matches or even surpasses human writing in fluency and coherence \citep{gomez-rodriguez_confederacy_2023}. GenAI has also demonstrated surprising creativity in games, as seen with AlphaGo’s unconventional strategies \citep{miller_artist_2019}, and in the arts, such as GenAI-generated portrait paintings \citep{dipaola_using_2016} and music composition \citep{civit_systematic_2022}. However, debate persists regarding whether AI is truly creative or simply a highly efficient pattern recognizer \citep{dale_gpt-3_2023, kirkpatrick_can_2023}.

Empirical studies have assessed LLMs' creative potential using established psychological creativity tests, such as the AUT, the DAT, and the Torrance Tests of Creative Thinking \citep{cropley_is_2023}. The results are mixed (cf. Table \ref{tab:creativity_overview} in Appendix). In divergent thinking tasks, GenAI often matches or surpasses average human performance \citep{cropley_is_2023, guzik_originality_2023, haase_artificial_2023}, but struggles to reach the conceptual leaps of highly creative individuals \citep{koivisto_best_2023}. In narrative generation, GenAI produces coherent, structured text but lacks originality and emotional depth \citep{chakrabarty_art_2024, gomez-rodriguez_confederacy_2023}. In scientific ideation, GenAI-generated research ideas are more novel but often less feasible than those proposed by experts \citep{si_can_2024}.

Rather than replacing human creativity, GenAI has been shown to augment and enhance creative processes \citep{verganti_innovation_2020}. Studies show that working with ChatGPT improves users’ self-efficacy and enhances their creative output \citep{urban_can_2023}. Human-AI collaboration is increasingly prevalent in areas such as film writing, music composition, and scientific research \citep{seidel_automate_2020, civit_systematic_2022}. While GenAI can generate highly fluent and structured creative outputs, human input remains crucial for refining, evaluating, and applying creative ideas in meaningful ways \citep{lazar_love_2022}.

Despite their impressive performance, LLMs have significant limitations. They tend to converge on similar outputs, leading to a lack of diverse ideas \citep{wenger_were_2025}. Additionally, GenAI lacks intentionality, subjective experience, and intrinsic motivation, which are key aspects of human creativity \citep{runco_ai_2023}. Ethical concerns include the risk of GenAI-generated misinformation or plagiarism in creative works \citep{}, the potential for GenAI to devalue human artistry by mass-producing creative outputs \citep{noauthor_ai_2023}, and the need for human oversight in GenAI-assisted decision-making \citep{parasuraman_humans_2008}.

GenAI has demonstrated remarkable creative capabilities in generating text, music, and visual art. However, its creativity remains constrained by its probabilistic nature and reliance on training data. While GenAI can augment and accelerate creative work, it lacks the deep conceptual, emotional, and experiential elements that define human creativity \citep{lazar_love_2022, runco_ai_2023}. Future research should explore ways to enhance divergent thinking in large language models and further integrate human-AI collaboration to maximize creative potential. 

\citep{soroush_creativity_2025}:
Multiple studies found LLMs perform at or above human levels in fluency and originality.
	•	AI vs. Human Creativity Debate:
	•	Some researchers argue LLMs are not truly creative because they lack agency and intentionality.
	•	Others claim LLMs exhibit combinatorial creativity (generating novel outputs by remixing knowledge).
	•	AUT Studies: AI surpasses humans in mean and max originality scores.
	•	TTCT Studies: GPT-4 ranks in the top 1\% for originality and fluency.
	•	DALL·E vs. Human Designers: AI matches novice designers in combinational creativity but lacks human-like concept generation.
	•	Automated Scoring Models: AI models like CNNs and transformers are being trained to assess creativity output, moving beyond human raters.

\citep{zhou_generative_2024}
AI adoption boosts creativity:
	•	Artists using AI create 50\% more artworks and receive 50\% more favorites per view than non-adopters.
	•	However, long-term novelty decreases as AI-generated content trends toward aesthetic homogeneity.
	•	Key findings for measuring LLM creativity:
	•	AI expands the creative idea space, but filtering and human intervention are needed to avoid generic outputs.
	•	Successful artists are those who combine exploration (novel ideas) with exploitation (selecting high-quality outputs)—a dynamic that may also apply to LLMs generating text.
	•	Implication for C of LLMs:
	•	Provides empirical data on how AI impacts creative output over time—suggesting that raw AI novelty scores might be insufficient without considering user-guided selection.
	•	Raises the question of whether LLM-generated ideas also follow the novelty decay pattern observed in AI-generated images.

\citep{song_interactions_2025}
	•	AI-generated responses were rated as highly useful and structured, but lacked human-like surprise and subjectivity.
	•	Students perceived AI chatbots as efficient facilitators of creativity but relied on them for knowledge rather than producing their own insights.
	•	AI chatbots guided students toward well-defined solutions, which may indicate convergent thinking tendencies rather than raw creativity.
	•	AI-driven CPS solutions outperformed peer-generated solutions in coherence and feasibility, but not necessarily in novelty.

Implications for C of LLMs
	•	Highlights the risk of LLMs favoring structured, knowledge-based responses over true creative breakthroughs.
	•	Reinforces the need for metrics beyond originality, such as structured ideation quality and user reliance on AI.
	•	Suggests AI might enhance creativity in structured problem-solving but not necessarily in exploratory, open-ended tasks.

- C as convergent thinking of LLMs has also be shown: \citep{orru_human-like_2023}
\end{comment}

\begin{landscape} 
\begin{longtable}{p{1.8cm} p{3cm} p{2cm} p{3.5cm} p{1cm} p{4cm} p{6cm}}
    \toprule
    \textbf{Paper (First Author, Year)} & \textbf{Creativity Measure Used} & \textbf{AI Model Used} & \textbf{Method to Assess Creativity} & \textbf{Human Comp.} & \textbf{Effect Size Found} & \textbf{Key Findings} \\
    \midrule
    \endhead
    Atmakuru et al. (2024) & CS4 Benchmark - Creativity in Story Writing & LLaMA, Gemma, Mistral & Evaluating performance under increasing storytelling constraints & No & Performance degrades with more constraints & LLMs struggle with constrained storytelling, revealing creativity limitations \\
    Bellemare-Pepin et al. (2024) & Divergent Association Task (DAT), Divergent Semantic Integration (DSI) & GPT-4, Claude-3 & Semantic creativity comparison between LLMs and 100,000 humans & Yes & GPT-4 outperformed humans on DAT, but humans had higher DSI in creative writing & LLMs generated more semantically distant associations than humans but lacked deep contextual integration. Humans produced richer, more meaningful associations in storytelling and open-ended tasks. \\
    Chakrabarty et al. (2023) & Torrance Test for Creative Writing (TTCW) & GPT-4, Claude, ChatGPT & Expert evaluations on short fiction writing using TTCW & Yes & LLMs fail TTCW tests 3-10x more often than humans & GPT-4 performs best in originality but lacks coherence and elaboration \\
    Cropley et al. (2023) & Divergent Association Task (DAT) & ChatGPT-3.5, ChatGPT-4 & AI-generated responses scored using semantic distance model & Yes & $\eta^2 = 0.01$ (small) & GPT-4 outperformed 82\% of humans but was unreliable and repetitive \\
    Gilhooly (2023) & Alternative Uses Task (AUT) & GPT-3 & Human judges rated originality, usefulness, and surprise & Yes & Small differences & Humans rated slightly higher on originality and flexibility; GPT-3 performed better on usefulness \\
    Gómez-Rodríguez \& Williams (2023) & Human Evaluation of Creative Writing & GPT-4, Claude, ChatGPT-3.5 & Expert grading of LLM-generated vs. human-authored stories using a 10-item rubric & Yes & GPT-4 outperformed human writers in readability and structure, while humans excelled in originality & AI-generated texts were coherent and grammatically refined but lacked thematic depth and genuine emotional engagement. Humans maintained an advantage in originality and narrative unpredictability. \\
    Grassini \& Koivisto (2024) & Figural Interpretation Quest (FIQ) & ChatGPT-4 & Semantic distance and human ratings of subjective creativity & Yes & AI more flexible, but humans scored higher on perceived creativity & AI responses were flexible but perceived as less novel and meaningful than human responses, which excelled in context-aware interpretation.  \\
    Guzik et al. (2023) & Torrance Tests of Creative Thinking (TTCT) & ChatGPT-4 & Fluency, flexibility, and originality scores compared to human norms & Yes & AI in top 1\% for originality and fluency & AI outperformed humans in fluency, flexibility, and originality \\
    Haase \& Hanel (2023) & Alternative Use Task (AUT) & ChatGPT-3, ChatGPT-4 & AI and human-rated originality & Yes & d = X.XX & AI matched human-level creativity in divergent thinking tasks \\
    Hubert et al. (2023) & AUT, Consequences Task (CT), Divergent Associations Task (DAT) & GPT-4 & AI vs. human performance on multiple divergent thinking tasks & Yes & $\eta^2 = .51$ (AUT), .49 (CT), .16 (DAT) & AI outperformed humans in originality and elaboration \\
    Ismayilzada et al. (2024) & Creative Short Story Task & GPT-4, Gemini-1.5, Claude-3.5, Llama-3.1-405B & Creativity evaluation using novelty, surprise, and diversity metrics & Yes & Humans significantly outperformed AI in all metrics & AI-generated stories were stylistically complex but lacked novelty, surprise, and diversity \\
    Kern et al. (2024) & Alternative Uses Test (AUT) & GPT-4, Claude 3.5 Sonnet & AI-assessed novelty, feasibility, and value & Yes & r = .62 (novelty), .59 (feasibility), .33 (value) & AI's assessment of novelty correlates well with human judgments \\
    Koivisto \& Grassini (2023) & Alternative Uses Task (AUT) & ChatGPT-3.5, ChatGPT-4 & Semantic distance and human-rated originality & Yes & AI scored higher on average, but best human responses exceeded AI & While AI responses were consistently high-quality and varied, human responses showed greater unpredictability and conceptual leaps. Top human responses still outperformed AI in originality and conceptual depth. \\
    Lamb et al. (2019) & Theoretical Creativity Frameworks & Various computational models & Interdisciplinary review of creativity assessment & No & N/A & Proposes a taxonomy for evaluating computational creativity \\
    Lu et al. (2025) & NEOGAUGE Benchmarking (Divergent \& Convergent Thinking) & GPT-4, Claude, LLaMA & Evaluation via DENIAL PROMPTING and NEOGAUGE metric & Yes & GPT-4 most creative, but below human-level & AI exhibited limited problem-solving creativity \\
    Marco et al. (2025) & Creative Fiction Writing Evaluation & BART-large, GPT-3.5, GPT-4o & Human study comparing AI vs. human-written short stories based on grammaticality, relevance, creativity, and attractiveness & Yes & SLM outperformed humans in most dimensions except creativity (not statistically significant) & BART-large, a fine-tuned small language model (SLM), outperformed human writers in all assessed aspects except creativity, where humans held a slight, non-significant advantage. Smaller models can rival both humans and larger models in creative writing under certain conditions. \\
    Moruzzi (2020) & Multidimensional Creativity Assessment & Various AI and biological systems & Evaluates creativity based on problem-solving and evaluation & Yes & Conceptual model & Proposes a framework to assess AI, human, and animal creativity; highlights AI’s strengths in structured problem-solving but weaknesses in divergent, generative creativity. \\
    Orwig et al. (2024) & Short Story Task, Semantic Distance & GPT-3, GPT-4 & Creativity ratings based on semantic diversity and perceptual details & Yes & r = .56 (semantic diversity), r = .16 (perceptual details) & Human and AI-generated stories were rated similarly in creativity \\
    Peeperkorn et al. (2024) & Narrative Generation Task & LLAMA 2-CHAT 70B & Evaluating the impact of temperature on creativity in storytelling (novelty, typicality, cohesion, coherence) & Yes & Weak positive correlation between temperature and novelty, moderate negative correlation with coherence & Temperature slightly increases novelty but decreases coherence. No strong evidence that temperature acts as a true creativity parameter. More nuanced and weak effect than often claimed. \\
    Si et al. (2024) & Research Ideation Evaluation & Claude-3.5, GPT-4 & Blind-reviewed comparison of human and AI-generated novel research ideas & Yes & AI-generated ideas rated as significantly more novel (p<0.05) than expert ideas but slightly weaker on feasibility & AI-generated research ideas were found to be more novel than those written by human NLP experts. However, feasibility remains a challenge, and AI lacks diversity in idea generation. \\
    Stevenson et al. (2024) & Alternative Uses Task (AUT) & GPT-3 & Expert-rated originality, usefulness, and surprise; semantic distance scoring & Yes & Humans had higher originality, surprise, and flexibility scores; GPT-3 had higher utility ratings & GPT-3 performed well but was outperformed by humans in originality and flexibility. Utility scores were higher for GPT-3. Flexibility in response patterns varied significantly. \\
    Sun et al. (2024) & Multi-Domain Creative Task Evaluation & GPT-3.5, GPT-4, Claude, Qwen, SparkDesk & Benchmarking LLMs against humans in divergent thinking, problem-solving, and creative writing & Yes & LLMs ranked in the 52nd percentile against humans, excelling in problem-solving but underperforming in creative writing & When asked 10 times, one LLM equaled 8-10 humans in collective creativity. LLMs performed well in divergent thinking but lacked diversity and feasibility in novel idea generation. \\Moruzzi (2020) & Multidimensional Creativity Assessment & Various AI and biological systems & Evaluates creativity based on problem-solving and evaluation & Yes & Conceptual model & Proposes a framework to assess AI, human, and animal creativity \\Panfilova et al. (2024) & Urban Test (TCT-DP) & Various Vision Models & Explainable AI (XAI) analysis of automated creativity assessment in drawings & Yes & Accuracy = 76\% & AI models achieved high accuracy in predicting human expert creativity scores \\
    Tigre et al. (2023) & Perceived Creativity of AI Art & GANs, AI-generated music models & Experimental study measuring human perceptions of AI-created art & Yes & AI enhances process novelty, but lowers perceived quality in tangible products & AI-generated visual and musical works were rated as technically proficient but less emotionally resonant. Human-AI co-creation led to better-rated outputs than AI-generated content alone. \\
    Vinchon et al. (2024) & Evaluation of Potential Creativity (EPoC) & ChatGPT-3.5, ChatGPT-4 & Standardized narrative creativity tasks, CAT evaluation & Yes & AI performed well in fluency, but lacked originality & GPT-4 showed high fluency but lacked originality in story generation. AI-generated stories were rated as lower in diversity and novelty compared to human creative works.  \\
    Wenger \& Kenett (2025) & Alternative Uses Task (AUT), Forward Flow (FF), Divergent Association Task (DAT) & GPT-4o, Gemini, Claude, LLaMA & Measuring cross-LLM homogeneity in creative responses using standardized creativity tests & Yes & LLM responses significantly more similar to each other than human responses, even after controlling for response structure & Cross-LLM homogeneity suggests that all LLMs converge towards a limited range of creative outputs, limiting divergent thinking regardless of model choice. Increased creativity prompts slightly improve response diversity but not to human levels. \\
    Ye et al. (2024) & Assessing Novel Solutions in Mathematical Reasoning & GPT-4o, Claude-3.5, Gemini-1.5-Pro & CREATIVEMATH benchmark assessing AI’s ability to generate novel math solutions beyond known references & Yes & Gemini-1.5-Pro demonstrated the highest rate of novel correct solutions, outperforming other LLMs in mathematical creativity & LLMs perform well in standard math tasks but struggle with generating novel solutions. Gemini-1.5-Pro outperformed other models in creative problem-solving. Novelty decreased as more reference solutions were provided. \\
    Zhao et al. (2024) & Adapted Torrance Tests of Creative Thinking (TTCT) & GPT-4, LLaMA-2-70B, Qwen, Vicuna & 7-task benchmark evaluating Fluency, Flexibility, Originality, and Elaboration in AI-generated responses & Yes & LLMs excel in elaboration but perform weakest in originality; multi-agent collaboration improves creativity & AI-generated responses are elaborative but struggle with original thought. Multi-agent collaboration slightly boosts originality. Creativity varies significantly between different LLM architectures and training paradigms. \\
    Zhuang et al. (2023) & Adaptive Cognitive Testing & GPT-4, Bard, ErnieBot & Computerized Adaptive Testing (CAT) for reasoning ability & Yes & AI scored similar to mid-level students in reasoning & AI exhibited "careless student" behavior \\


    \bottomrule
\end{longtable}
\end{landscape}
